Enhancing the hunt for new phenomena in dijet final-states using anomaly detection filters at the High-Luminosity Large Hadron Collider

In the realm of dijet searches in high-energy physics, a significant challenge has emerged: with experiments producing more and more data, the traditional methods of using analytic functions to describe dijet mass spectra start to fail. To address this, we suggest the application of an anomaly detection approach to eliminate less interesting background events based on event final states. This method not only bypasses the limitations of conventional background models but also significantly enhances our ability to detect potential signals of new physics. Through simulations that mimic the conditions of the upcoming High-Luminosity Large Hadron Collider, we demonstrate the strength and efficiency of this approach in dealing with large data volumes. The integration of unsupervised machine learning into our experimental framework paves the way for a promising avenue to unveil hidden physics discoveries within the overwhelming influx of data.

==> Makefile <==
###############################################################################
#
# Makefile for the photon note
#                              	
###############################################################################

NOTENAME=main

all:#default target makes everything
	pdflatex $(NOTENAME).tex && bibtex $(NOTENAME) && pdflatex $(NOTENAME).tex && pdflatex $(NOTENAME).tex

dvi:
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex 

ps:
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex && latex $(NOTENAME).tex && dvips -P pdf $(NOTENAME).dvi 

pdf:
	latex $(NOTENAME).tex && bibtex $(NOTENAME) && latex $(NOTENAME).tex && latex $(NOTENAME).tex && dvips -P pdf $(NOTENAME).dvi && ps2pdf $(NOTENAME).ps $(NOTENAME).pdf

show:
	evince $(NOTENAME).pdf

.PHONY: clean
clean:
	rm -rf $(NOTENAME).aux $(NOTENAME).log $(NOTENAME).out $(NOTENAME).blg $(NOTENAME).fdb_latexmk $(NOTENAME).fls $(NOTENAME).spl \
	$(NOTENAME).dvi $(NOTENAME).ps \
	$(NOTENAME).toc $(NOTENAME).tof thumb*.* *~ 

